Conflict-Based Search for Connected Multi-Agent Path Finding

We study a variant of the multi-agent path finding problem (MAPF) in which agents are required to remain connected to each other and to a designated base. This problem has applications in search and rescue missions where the entire execution must be monitored by a human operator. We re-visit the conflict-based search algorithm known for MAPF, and define a variant where conflicts arise from disconnections rather than collisions. We study optimizations, and give experimental results in which we compare our algorithms with the literature.

==> sec_discussion.tex <==

%In the work of Boyarski et al.~\cite{Boyarski:15:ICBS}, the authors suggest to
%prioritize the cardinal conflicts in an execution.
%This optimization prevents
%the algorithm to generate a large sub-tree below a node with the same cost.
%Additionally, the cardinal conflict will eventually reappear lower until it is
%solved.

% In order to detect cardinal conflicts without generating all children, Boyarski et
% al.~\cite{Boyarski:15:ICBS} use multi-valued decision
% diagrams (MDD) to represent the set of all paths for an agent to reach its
% goal in a given number of steps. These were introduced in~\cite{Sharon:11:ICT}.

% An \emph{MDD} for an agent $\vAgent$ for $k$ steps starting at $s$ to reach $g$,
% denoted $MDD_\vAgent^k$ is a Directed Acyclic Graph (DAG) with a single root node
% ($s$) and sink node ($g$). We depict an example of an MDD in
% Figure~\ref{fig:MDD}.

%\begin{figure}
%	\centering
%	\begin{tikzpicture}[shorten >=1pt,->, rotate=90, yscale=1.5, xscale=0.8]
%		\tikzstyle{vertex}=[circle,fill=black!15,minimum size=17pt,inner sep=0pt]
%		\node[vertex] (root) at (1,5) {$s$};
%
%		\node[vertex] (v1) at (0,4) {$v_1$};
%		\node[vertex] (v2) at (2,4) {$v_2$};
%
%		\node[vertex] (v3) at (0,3) {$v_3$};
%		\node[vertex] (v4) at (1,3) {$v_4$};
%		\node[vertex] (v5) at (2,3) {$v_5$};
%
%		\node[vertex] (v6) at (1,2) {$v_6$};
%
%		\node[vertex] (sink) at (1,1) {$g$};
%
%		\draw (root) -- (v1);
%		\draw (root) -- (v2);
%
%		\draw (v1) -- (v3);
%		\draw (v1) -- (v4);
%		\draw (v1) -- (v5);
%		\draw (v2) -- (v5);
%
%		\draw (v3) -- (v6);
%		\draw (v4) -- (v6);
%		\draw (v5) -- (v6);
%
%		\draw (v6) -- (sink);
%	\end{tikzpicture}
%	\caption{Example of an MDD from $s$ to $g$ using $4$ steps.}
%	\label{fig:MDD}
%\end{figure}

% $MDD_\vAgent^k$ can be built from a sub-graph resulting from a breath-first search
% starting at the start location of agent $\vAgent$ and stopped at depth $k$. From $MDD_\vAgent^k$, one can easily compute $MDD_\vAgent^{k+1}$. Furthermore, given a set of constraints
% $\sConstSet$ over the path of an agent, one can decide the existence of a path
% for agent $\vAgent$ in $k$ steps satisfying $\sConstSet$ in linear-time over the MDD.
% One can thus check if a conflict is cardinal in linear-time on the size of the MDD.


% \subsection{Conflict Prioritization}
% A conflict at node $\vNode$ is said to be
% $i$-\emph{cardinal} if $\vNode$ has $i$ child nodes $\vNodeChild$ with
% $\vNodeChild.\vCost > \vNode.\vCost$. We call a $\vAgentsNumber$-cardinal
% conflict simply a \emph{cardinal} conflict and a $0$-cardinal conflict a
% \emph{non-cardinal} conflict.

% We use this notion \todo{laquelle?} to prioritize conflicts to split when considering a node in
% the constraint tree. At each chosen node, we split a $i$-cardinal conflict with the largest~$i$. 

% This is a generalization of the prioritization introduced in~\cite{Boyarski:15:CBSBP}.
% In the latter work, conflicts involve the collision of two agents, and using our terminology, the authors prioritize $2$-cardinal conflicts over other conflicts.
% Our generalization allows us to refine this prioritization, which applies well to connectivity conflicts.

% Note that no overhead is created from this optimization as all conflicts must be solved anyway. Nonetheless, the order in which the conflicts are solved is important and this is what reduces the number of expansions done in the constraint tree, hence its size.



==> sec_theory.tex <==
\begin{definition}
    We denote $OPT(n)$ for a node $n$, the optimal valid execution satisfying
    the constraints $n.c$.
\end{definition}

\begin{lemma}
    For all node $n$,  $n.cost \leq |OPT(n)|$.
    \label{lem:admi}
\end{lemma}

\begin{proof}
    From a node $n$, $n.cost$ is the cost of the current execution. If the
    current execution is valid, then $n.cost = |OPT(n)|$. If the current
    execution is not valid, then an additional constraint will extend the path
    of an agent, thus $n.cost < |OPT(n)|$, or only change the position of an
    agent along its path, thus $n.cost = |OPT(n)|$.
\end{proof}

\begin{lemma}
    If an execution $e$ is valid then there exists a node $n$ in OPEN which
    allows $e$.
    \label{lem:compl}
\end{lemma}

\begin{proof}
    This lemma is shown by induction on OPEN. At the beginning, the root is not
    constrained, thus $e$ is allowed. Let us assume that it is true after $i$
    steps. Then, the nodes $m_1, \dots, m_k$ are generated. Knowing that $e$ is
    valid from $n$, then it must satisfy at least $n.c$ and one of $m_i.c$.
\end{proof}

\begin{theorem}
    \sAlgo returns an optimal solution.
\end{theorem}

\begin{proof}
    Whenever a goal node $g$ is generated all valid executions are permitted by
    $g.c$ (Lemma~\ref{lem:compl}). Knowing that $g$ is a goal node, then $g.cost
    \leq |OPT(g)|$ (Lemma~\ref{lem:admi}). Furthermore, the node extracted from
    OPEN is the one which minimizes the cost.
\end{proof}

